PartAL: Efficient Partial Active Learning in Multi-Task Visual Settings

Multi-task learning is central to many real-world applications. Unfortunately, obtaining labelled data for all tasks is time-consuming, challenging, and expensive. Active Learning (AL) can be used to reduce this burden. Existing techniques typically involve picking images to be annotated and providing annotations for all tasks. In this paper, we show that it is more effective to select not only the images to be annotated but also a subset of tasks for which to provide annotations at each AL iteration. Furthermore, the annotations that are provided can be used to guess pseudo-labels for the tasks that remain unannotated. We demonstrate the effectiveness of our approach on several popular multi-task datasets.

==> bib/figmacro.tex <==
\newif\ifrgb
\rgbfalse

\newif\iffig
\figtrue

\newcommand{\figx}[2]
{
 \iffig
  \includegraphics[width=#1,keepaspectratio]{#2} 
 \else
   \parbox{#1}{#2} 
 \fi
}

\newcommand{\figy}[2]
{
 \iffig
  \includegraphics[height=#1,keepaspectratio]{#2}  
   \else
  \parbox{#1}{#2} 
 \fi
}

\newcommand{\figxy}[3]
{
 \iffig
  \includegraphics[width=#1,height=#2]{#3} 
 \else
   \parbox{#1}{#2}
  \fi
}

\newcommand{\figurecaption}[2]
{
\caption[]{\parbox[t]{#1}{#2}}
}

\newcommand{\fcaption}[1]
{
 \figurecaption{0.9\linewidth}{\small #1}
}

\newcommand{\figdir}[1]
{
\def\figurepath{#1}
}

\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{.0}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}


==> bib/report.tex <==
\usepackage{named}

\usepackage{geometry}
\usepackage{times}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsthm,amssymb}
\usepackage{color}

\geometry{
 a4paper,
 left=21mm,
 right=21mm,
 top=16mm,
 bottom=16mm,
 }
 
%\setlength{\oddsidemargin}{0.0in}
%\setlength{\topmargin}{-0.125in}
%\setlength{\textwidth}{6.25in}
%\setlength{\textheight}{8.75in}
%\parskip 6pt plus 3pt minus 2pt

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\im}{\item}
\newcommand{\comment}[1]{}
\newcommand{\missing}[1]{\begin{large} {\bf ADD:} {\em #1} \end{large}}
\newcommand{\note}[1]{\begin{center} \noindent\framebox{\begin{minipage}{8cm}{\bf #1}\end{minipage}}\end{center}\\}
\newcommand{\rmk}[1]{{\color{red}{ \bf #1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\url}[1]{#1}

\newif\ifsubmit
\submitfalse

\newif\ifdraft
\draftfalse

\newcommand{\dspace}{\renewcommand{\baselinestretch}{1.5}\large\normalsize}
\newcommand{\sspace}{\renewcommand{\baselinestretch}{1.0}\large\normalsize}
\newcommand{\Section}[1]{\section{#1}}
\newcommand{\SubSection}[1]{\subsection{#1}}
\sspace

\renewcommand{\floatpagefraction}{1.0}


==> fig/inference.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.47\textwidth]{images/improved_inference.pdf}
    %\includegraphics[width=0.98\textwidth]{images/PADNet.pdf}
    % \vspace{-4mm}
    \caption{\small {\bf Improving inference with available labels.} Given a single RGB image and available ground truth targets as an input, we modify PAD-Net to reuse available modalities to improve accuracy of final predictions. Combining both predicted intermediate prediction (red) and actual ground truths (green), we pass them further into Multi-Modal Distillation block to generate final prediction.}
    \label{fig:improved-inference}
\end{figure}


% produces a set of intermediate predictions that are fed to a distillation module. The output is a final set of predictions that pool information from all modalities. The $\mathcal{L}_{i}$ represent losses for intermediate and final predictions that are used at training time. At inference time, it is possible to replace some of the intermediate predictions by ground-truth images if they happen to be available

==> fig/mtask.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[h!]
    \includegraphics[width=0.85\textwidth]{images/padnet_mod.pdf}
    \centering
    \caption{
    \textbf{\pale{}'s improved multi-task inference.} Given a multi-modal sample with partially labelled targets, our method utilises available modalities in order to infer the rest and make decisions about labelling separately for each of these absent targets.
    }
    \label{fig:mtask}
\end{figure}

==> fig/pseudo.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
    \includegraphics[width=0.5\textwidth]{images/pseudo_labelling.pdf}
    \centering
    \vspace{-7mm}
    \caption{
    \textbf{Sharing information across tasks.} \pale{}  exploits the correlations between modalities to extract additional information during training. In this example depths labels can be used to predict normals, which are then used as additional labels or pseudo-labels.    }
    \label{fig: pseudo}
\end{figure}

